Energy-Aware Neural Architecture Optimization with Fast Splitting Steepest Descent

Designing energy-efficient networks is of critical importance for enabling state-of-the-art deep learning in mobile and edge settings where the computation and energy budgets are highly limited. Recently, Liu et al. (2019) framed the search of efficient neural architectures into a continuous splitting process: it iteratively splits existing neurons into multiple off-springs to achieve progressive loss minimization, thus finding novel architectures by gradually growing the neural network. However, this method was not specifically tailored for designing energy-efficient networks, and is computationally expensive on large-scale benchmarks. In this work, we substantially improve Liu et al. (2019) in two significant ways: 1) we incorporate the energy cost of splitting different neurons to better guide the splitting process, thereby discovering more energy-efficient network architectures; 2) we substantially speed up the splitting process of Liu et al. (2019), which requires expensive eigen-decomposition, by proposing a highly scalable Rayleigh-quotient stochastic gradient algorithm. Our fast algorithm allows us to reduce the computational cost of splitting to the same level of typical back-propagation updates and enables efficient implementation on GPU. Extensive empirical results show that our method can train highly accurate and energy-efficient networks on challenging datasets such as ImageNet, improving a variety of baselines, including the pruning-based methods and expert-designed architectures.

==> tex/intro_old.tex <==
\section{Introduction}

% In recently years, deep neural networks have achieved significant empirical success in various domains. When applying deep learning to the task at hand, the optimal deep-net architecture might reasonably be expected to depend on the learning task that is being considered.
% Though there have been rapid progresses for automatic deep-net architectures optimization recently, such as neural network architecture search (NAS) and network pruning etc., designing the best architectures still requires a lot of expert knowledge and trial-and-errors.


% % This work is a follow-up of our previous submission (done in UT Austin) to Neurips 2019, which introduces a progressive learning strategy that allows us to incrementally grow a network with theoretical advantages. The overall process works by splitting the existing neurons into multiple copies by leveraging a functional gradient descent idea. We derived a simple criterion, which is referred as splitting index, for deciding the best subset of neurons to split. The neurons ranked top are splitting into two off-springs following a splitting gradient direction.

% To calculate the splitting index, one needs to compute the minimum eigenvalues of splitting matrices. The computational cost of evaluating all the splitting indexes is $O(nd^3)$, where n is the number of neurons (e.g. conv filters) and d is the number of parameters of each neuron. For large-scale deep-networks, the dimension d could be large (e.g., $d = c*k*k$, where c is the number of input channels and k is the kernel size), we might not be able to analytically compute the splitting indexes in practice.  As a key contribution of this work; we propose a gradient-based efficient approximation to estimate the splitting indexes by minimizing the Rayleigh quotient. The gradient of the Rayleigh quotient, however, which involves in computing multiplication between a high dimensional splitting matrix and a vector. A key observation is that, the computation can be easily automated using automatic differentiation tools by constructing an auxiliary function with careful design. This approach allows us to quickly implement and grow the network with little effort.

% The aforementioned approach grows the network that only focusing on empirical loss minimization while neglecting the different energy consumption level of different neurons. Intuitively, one may consider using less neurons in shallow layers which have larger input resolution and consume more energy in general; on the other hand, one should retain more neurons in deep layers which are responsible for final classification and computational cheap.

% The splitting strategy contributes to the final accuracy and energy efficiency of neural architectures in a complex manner. We further propose an energy-aware splitting mechanism that allows us to learn more computation-efficient networks, which is of critical importance for resource-constrained settings such as mobile devices and edge devices.

%Deep learning with over-parameterized networks
Deep neural networks (DNNs)
has demonstrated remarkable performance in solving
various challenge problems such as image classification, object detection
and language understanding. 
Although large-scale deep networks have good empirical properties, 
their large sizes 
cause slow computation and high energy cost in the inference phase.
% As a result, 
% their applications are largely limited by the high computational complexity and energy costs,
% % prohibitive computational overhead, 
% 
This imposes a great challenge for 
%the broader 
improving the applicability of deep networks to more real-word domains, 
%due to inference inefficiency, 
% The high computational complexity and energy costs of deep-nets impede their broader applicability, 
especially on mobile and edge devices where the computation and energy budgets are highly limited.

% Though there have been rapid progresses for automatic deep-net architectures optimization recently, such as neural network architecture search (NAS) and network pruning etc., designing the best architectures still requires a lot of expert knowledge and trial-and-errors.

% On the large scale iamgenet dataset,
% we method achieves xx top-1 accuracy that yields xxx improvement while maintaining the
% same number of FLOPS per inference using MobilenetV1. XXXX\red{todo}
 
% \red{fix later}
% In this work,
Recently, \citet{splitting2019} proposes 
% we extends a recently proposed  
a novel  splitting steepest descent approach for neural architecture optimization. 
Instead of treating architecture search as a discrete 
(or with continuous relaxation) optimization problem \citep[e.g.][]{li2016pruning, liu2017learning, cai2018proxylessnas}, 
% \citet{splitting2019} formulates the architecture search problem as a continuous functional optimization problem in the space of the distributions of the neurons. 
% The functional splitting steepest
% descent mimics the typical gradient updates but enables exploration in the architecture space without approximation.
The final algorithm is simple, 
which alternates between a standard parametric
gradient descent phase to reach a parametric local minima,
and a splitting phase in which a subset of neurons is chosen to split according 
to a so-called splitting-index that gives the optimal improvements.
% we grow
% the network by splitting existing neurons into several off-springs.



However, the aforementioned approach grows the network that only focusing on empirical loss minimization while neglecting the different energy consumption level of different neurons. 
The splitting strategy contributes to the final accuracy and energy efficiency of neural architectures in a complex manner. We propose an energy-aware splitting mechanism that allows us to learn more computation-efficient networks, which is of critical importance for resource-constrained settings such as mobile devices and edge devices.


Moreover, 
to calculate the splitting index,
one needs to compute the minimum eigenvalues of splitting matrices.
The overall splitting process is often computational expensive for modern 
neural networks with thousands neurons.
As a key contribution of this work; we propose a gradient-based efficient approximation to estimate the splitting indexes by minimizing the Rayleigh quotient. This approach allows us to quickly implement and grow the network with little effort.

Empirically, our method discovers novel networks that more accuracte
when targeting similar flops-constrains on the Cifar100 benchmark dataset compared with strong pruning baselines \citep[e.g.][]{liu2017learning, li2016pruning, gordon2018morphnet}.
On the large-scale ImageNet dataset, our method outerforms strong baselines \citep{he2018amc, howard2017mobilenets, sandler2018mobilenetv2}, 
archives 73.98\% and 72.84\% top-1 accuracy using MobileNetV1 \citep{howard2017mobilenets} and MobileNetv2 \citep{sandler2018mobilenetv2}, respectively.
The gain is even more significant on the low-flops regime. 

==> tex/splitting_old.tex <==
\section{Splitting steepest descent for neural architecture optimization}
% We introduce the background of splitting steepest descent, which forms the foundation of
% our work.
Our work builds upon a recently proposed splitting steepest descent idea \citep{splitting2019} 
for progressively training 
deep neural networks.
% for neural architecture optimization.


\begin{figure*}
\centering
\begin{tabular}{ccc}
\setlength\tabcolsep{1pt}
\hspace{-0.5em}
\includegraphics[width=0.26\textwidth]{figures/net_split_new.png} &
\hspace{-0.2em}
\includegraphics[width=0.32\textwidth]{figures/splittingcurve_new.png} & 
\hspace{-1.2em}
\includegraphics[width=0.35\textwidth]{figures/splitting-idea-new.png} 
\\
 (a) %Neuron splitting & 
 & (b) & 
 (c) %Monotone improvements \\
\end{tabular}
\caption{
(a) Splitting one neuron into two off-springs.  
(b) Steepest descent on the overall architecture space 
consists of both standard gradient descent on the parameters (with fixed network structures), and updates of the network structures (via splitting). % across the boundaries of different network structures. 
%The structural update allows us to escape the local optima when training with a fixed structure, by jumping into a higher dimension (via splitting neurons). 
(c) The local optima in the low dimensional space 
is turned into a saddle point in a higher dimensional of the augmented networks, and hence can be escaped by our splitting strategy, yielding monotonic decrease of the loss. % via stochastic 
%of our splitting process for architecture optimization. 
%(b) Jumping into a higher dimensional parameter space allows us to escape local minima;
%(b) splitting a  neuron into two copies; 
%(c) progressive training via splitting yields monotone improvements.
}
 \label{fig:intuition}
\vspace{-1em}
\end{figure*}


% Consider a neural network with one neuron, (stochastic) gradient descent is often applied to learn the optimal network parameters. However,  gradient  descent  can  only  yield  parametric  updates  of  model  parameters. At a stable local minima, the first order gradients become zero and no further improve can be made. In order to further reduce the loss, we propose to generalize the optimization to a higher-dimensional parameter space (e.g. 2, see Figure 2). With the additional freedom, the previous stationary point may turn into a saddle point in the new augmented parameter space, one could decrease the loss again by running(stochastic) gradient descent with small perturbations.

% Intuitively,  the  1-dimensional  case  corresponds  to  a  neural  network  with  one  neuron;  while  the higher-dimensional case relates to neural network optimization with more neurons.  In the context of neural architecture optimization, our generalization allows to grow the network naturally by ex-tending the low-dimensional parametric optimization to a higher-dimensional space, which yields monotonic improvements without degradation.  Theoretically, this can be viewed as a second or-der descent for escaping saddle points in the functional space while the parametric gradient descent corresponds to a first order descent.

% \begin{align*}
% \min_z ~~\gL(\Phi(\rho, z)) - \gL(\rho) \\
% \text{s.t.}~~\sum z \le c\\
% z_i \in \{0, 1\} ~~\forall i \\
% \end{align*}

% We aim at searching resource-efficient neural architectures. 
% To be concrete, 
% \begin{align*}
% \min_{\alpha \in \mathcal{A}} ~\min_{\Theta(\alpha)} \gL(\alpha, \Theta(\alpha)) \\
% R(\alpha) < \tau.
% \end{align*}
% Given a network architecture $\alpha$, 
% $\Theta(\alpha)$ is the model weights associated with the network. $\gL(\cdot)$ stands for the loss
% function.
% $R(\alpha)$ measures the energy consumption
% yields by the network $\alpha$. 
% The goal is to find the best architecture and model parameters satisfies the resource constrain that  achieving the minimum loss.

% % We use one layer neural network as a motivation example,

% Given an observation dataset 
% $\D = \{x_i\}_{i=1}^n$
% the  model parameters are learned by minimizing a loss funciton
% with $\Theta= \{\theta_i\}_{i=1}^m$,
% $$
% \gL(\Theta; \D) = \frac{1}{n} \sum_{i=1}^n \bigg[
% \bigg]
% $$

% \red{quick versio, rewrite later}
\paragraph{Motivation example}



Our key idea is to view neural architecture search as a continuous optimization in the configuration space of the neuron parameters, on which steepest descent can be introduced for efficient optimization. 
%To illustrate the idea,  consider  one-hidden-layer neural networks, which are 
To fix the idea, assume the neural network structure is specified by a set of size parameters $\vv m= \{m_1,\ldots, m_K\},$ where each  $m_k$ could denote the number of neurons of in the $k$-th layer, or of the $k$th type. 
Denote by $\Theta_{\vv m}$ 
the parameter space of  networks of size $\vv m$, 
%$\{\theta_i\}_{i=1}^m$, 
then $\Theta_\infty = \cup_{\vv m\in \mathbb{N}^K} \Theta_{\vv m}$, called the  configuration space, is the space of all possible neural architectures and parameters.  

In this view, learning parameters for a fixed network  
is minimizing the loss inside  an individual sub-region  $\Theta_{\vv m}$, % with a fixed size $m$, 
while optimizing in the overall configuration space $\Theta_\infty$ admits the co-optimization of both the architecture and parameters. 
The key observation is that by considering optimization on $\Theta_\infty$ (instead, e.g., on the discrete size parameters $\vv m$), 
we obtain an (infinite dimensional)  continuous optimization on $\Theta_\infty$. 
With a proper definition of distance on $\Theta_\infty$, % with a proper notion of distance, 
  we can then derive generalized steepest descent on $\Theta_\infty$ 
  that leverages valuable gradient information %(a.k.a. gradient) 
 to optimize the architectures more efficiently.  
%, as we discover in our derivation,  

Intuitively, the steepest descent on $\Theta_\infty$ should consist of two phases:  
1) the steepest descent inside each $\Theta_{\vv m}$ with a fixed $\vv m$, which 
 reduces to the standard gradient descent on parameters, % descent inside each $\Theta_m$ fixed $m$,
 and 2)  the descent across the boundary of different sub-regions $\Theta_{\vv m}$, which corresponds to optimal updates 
 on the network structures. 
 %structural
 %when transferring between different sizes. 
%it is possible to definen 
%Critically, as we 
%while architecture search admits an optimization on the overall configuration space $\Theta_\infty$, which requires the joint optimization of size $m$ and the parameters. 
%Motivate by 
%It is this view that allows us to conquer NAS with gradient descent by mathematical deriving steepest descent algorithms in the configuration spface $\Theta_\infty$. Our novel steepest descent $\Theta_\infty$ shall reduce to the standard parametric gradient descent inside each $\Theta_m$ fixed $m$, while introducing novel structural updates when transferring between different sizes. 
%Intuitively, 
The structural descent across boundaries of $\Theta_{\vv m}$ 
%Our view can also be understood from
can be viewed  %the perspective of  
as escaping saddle points in the configuration space. 
As shown in Figure~\ref{fig:intuition}(b),  
when the parametric training inside a fixed $\Theta_{\vv m}$ gets saturated, 
%augmenting the network 
structural descent allows us to escape local optima by jumping into a higher dimensional sub-region. 
The idea is that the local optima inside $\Theta_{\vv m}$ can be turned into a saddle point in the higher dimensional configuration space $\Theta_{\vv m}$ (Figure~\ref{fig:intuition}(c)), 
which can be escaped easily using stochastic gradient descent on the higher dimensional space. 


% A key observation is that, 
Figure~\ref{fig:intuition} highlights a key observation of the neuron splitting idea 
for neural architecture optimization.
When the typical first order parametric updates get stuck, 
% one might perform to escape the local minima.
one might consider generalizing the optimization
to a higher-dimensional parameter space.
% to escape the local minima.
With the additional freedom, the previous local minimum might turn into
a saddle point in the new parameter space. In this way, one would be able to
decrease the loss further by continually 
running stochastic gradient descent (SGD).
In the context of
neural architecture optimization, 
the mapping from a lower-dimensional space to a higher-dimensional parameter space 
corresponds to grow the network via introducing more trainable neurons.
% higher-dimensional parametric updates correspond to optimize a larger network, 
% thus allowing us to exploring the architecture space implicitly. 
% thus yielding monotonic improvements without degradation.


\paragraph{Escaping local minima via splitting}
% It remains to show how to achieve the generalization.
\citet{splitting2019} showed that the aforementioned generalization could be achieved simply
by splitting existing neurons into multiple copies.
Specifically, 
consider a network with one neuron $w$, 
% let $\sigma(\theta, x)$ be a neuron and $\theta$ its parameters and $x$ the input, 
assume the loss has a form,
$$
\gL(w) := \E_{x\sim \gD}[\gM(\sigma(w, x))],
$$
where $\gD$ is a collection of training data, $\sigma(w, x)$ represents the activation function and $\gM$ defines the loss given input $x$.
% the network which is determined 
% by the overall loss function.
% and $\Phi$ is the map deterined by the oveall loss function.
% To extend the lower dimensional parameter space to a higher diemsnional space
% Intuitively, the low dimensional case corresponds to a neural network with one neuron; while the higher-dimensional case relates to network optimization with more neurons.
%  As we can see from the previous example,
% it’s useful to 
% split existing neurons to multiple copies
% introduce more neurons at a stable local minima 
% in order to achieve additional improvements. 
% In practice, this would be implemented via splitting neurons into multiple copies. 
% In practice, this could be implemented via splitting neurons into multiple copies. 
Consider splitting neuron $w$ into $m$ off-springs $\{w_i\}_{i=1}^m$
associated with weights $\{z_i\}_{i=1}^m$, hence 
the new augmented loss could be written as follows
$$
\gL(\{w_i, z_i\}) = \E_{x\sim \gD}\bigg[ \gM\bigg(\sum_{i=1}^m z_i \sigma_i(w_i, x)\bigg) \bigg].
$$
It is easy to see that the splitting-induced network and loss are equivalent to the original loss
such  that $\gL(\{w_i, z_i\}) = \gL(w)$  when $w_i = w$ and $\sum_{i=1}^m z_i = 1$.
As shown in \citet{splitting2019},
a key property of this construction
is that it introduces a smooth change on the loss function
without destroying the optimization states. 
the smooth change allows us to derive the splitting strategies to achieve the maximum loss decrease  when perturbing all off-springs within a infinitesimal neighborhood, 
as we introduce in the sequel.

% $\{\theta_i\}$ defines a larger network with $m$ neurons. 

% To set up the notations, 
\paragraph{Deriving optimal splitting solutions}
Without loss of generality, 
consider a deep neural network with 
a collection of neurons $\Theta = \{\theta^{[1]}, \cdots, \theta^{[n]}\}$.
% For example,  
In the case of convolution layer,
% $m_\ell$ represents the number of output channels and 
each neuron $\theta^{[i]}$ represents a convolution filter with dimension $n_{in}\times k^2$,
with $n_{in}$ is the number of input channels and $k$ denotes
the kernel size. 

% Given a set of training examples $\gD = \{ (x, y)\}$. 
To learn the optimal
network parameters, we train the network by minimizing the empirical loss,
$$
\gL(\Theta) := \E_{x\sim \gD}\bigg[ \gM(\sigma(\theta^[\ell], g(x; \theta^{[\neg \ell]})); \theta^{[\neg \ell]})\bigg],
$$
Similarly, 
let $\gM(\cdot)$ as a function determined by the overall loss and $g(\cdot)$ 
be the input of neuron $\theta^{[\ell]}$.
% where $\gM(x,\Theta)$ maps 
Our goal is to split neurons into off-springs
and perturb them in an infinitesimal neighborhood 
such that the training loss is maximamly decreased in the new parameter space. 
% xx achieves by splitting existing neurons into multiple copies. 
To be precise, considering split each neuron $\theta^{[\ell]} \in \Theta$ 
into $m$ off-springs $\{w_i^{[\ell]},~\theta_i^{[\ell]}\}_{i=1}^m$, 
where $\{w_i\}$ is set of weights associated with each copies. 
% It is easy to shown that
Let $\gS\cdot \Theta$ represent the network induced via splitting.
Similar to the one neuron case, we have
$
\gL(\gS \circ \Theta) = \gL(\Theta)
$
when $\sum_{i=1}^m w_i^{[\ell]} =1$ and $\theta_i^{[\ell]} = \theta^{[\ell]}$.

To achieve improvements, we update all off-springs with small 
perturbations following
$$
\theta_i^{[\ell]} = \theta^{[\ell]} + \epsilon(\mu^{[\ell]} + \delta_i^{[\ell]}),
$$
where $\epsilon$ is a small step size and $\delta_i^{[\ell]}$ denotes the 
individual splitting direction and $\mu^{[\ell]}$ is
the average perturbation shared by all off-springs. 
% For each neuron $\theta^{[\ell]}$, 
The key problem is to find the optimal splitting strategies  
to decrease the loss between the 
$\gL(\gS\circ \Theta)$ and $\gL(\Theta)$ as fast as possible.
This can be solved by following the observation shown in \citet{splitting2019}, 
\begin{align}
\min_{m, \{w_i^{\ell}, \delta_i^\ell \}} \bigg\{ \gL(\gS\circ\Theta) - \gL(\Theta) := \frac{\epsilon^2}{2} \sum_{\ell=1}^n \sum_{i=1}^m w_i^{[\ell]} {\delta_i^{[\ell]}}^\top S(\theta^{[\ell]}) \delta_i^{[\ell]} + \gO(\epsilon^3) \bigg\},
\label{eq:splitting}
\end{align}
where $S(\cdot)$ is the so-called splitting matrix, 
which has a form
$$
S(\theta) =  \E\bigg[ \nabla_\sigma \Phi\bigg( \sigma(\theta^{[\ell]},
g(x; \theta^{[\neg \ell]})); \theta^{[\neg \ell]}\bigg)  \nabla_{\theta\theta}^2 \sigma(\theta^{[\ell]},
g(x; \theta^{[\neg \ell]}) )\bigg].
$$
% Let $\gF(\theta^{[\ell]}) = \sum_{i=1}^m w_i^{[\ell]} {\delta_i^{[\ell]}}^\top S(\theta^{[\ell]}) \delta_i^{[\ell]} $ denote the splitting gain via splitting neuron $\theta^{[\ell]}$,
Therefore, the splitting effects of different neurons can be compared separately
without considering the other neurons,
the overall loss decrease caused by splitting is 
simply the sum of the individual splitting gains.
% allowing us to decide the best
% subset of neurons to split when a maximum number constrain is imposed.
It remains show the optimal solution of $\{m, w_i^{[\ell]}, \delta_i^{[\ell]}\}$ 
for Eq.~\eqref{eq:splitting}, 
for which the optimization has a closed form solution. The overall gain via splitting is
\begin{align}
\min_{m, \{w_i^{\ell}, \delta_i^\ell \}} \bigg\{ \gL(\gS\circ\Theta) - \gL(\Theta) \bigg\} =
\frac{\epsilon^2}{2}  \sum_{\ell=1}^n \lambda_{\min}(S(\theta^{\ell})),
\label{eq:loss_decrease}
\end{align}
where $\lambda_{\min}(S)$ is the minimum eigenvalue of the splitting matrix $S$.
% This gives the optimal splitting strategies. 
The corresponding optimal splitting strategies are as follows,
% The optimal solution of xx has been shown to to be $F = xx$,
% where 
$$
m = 2, w_1^{[\ell]} = w_2^{[\ell]} = 1/2, ~~~\delta_1^{[\ell]} = v_{\min}(S), ~~\delta_2^{[\ell]} = -v_{\min}(S), ~~~\forall \ell,
$$
with $v_{\min}(S)$ as the the eigenvector related to the minimum eigenvalues of the 
splitting-matrix $S$. 
% and the minimum value of 


% In this case, the optimal solution of Eq.~\eqref{xx} reduces to 
% $$
% \min_{m w_i, \delta_i} \bigg\{ \gF() := \sum_xx \bigg\}
% $$
%  xxx showed that the optimal solution of xxx is,
% where 

\paragraph{Implicit neural architecture optimization via splitting}
The splitting process allows us to grow the network via splitting
thus yielding a framework for implict neural architecture space exploration.
Given a budget of growing the network with $c$ neurons, we should choose the
the best subset of neurons that maximize the decrease loss.
The splitting effects of different neurons can be compared using the optimal
individual gain (see Eq.\eqref{eq:loss_decrease}) without considering the other neurons.
% allowing us to decide the best
% subset of neurons to split when a maximum number constrain is imposed.

To be precise, for a neural network with $m$ neurons, let $\vv\beta \in \R^n$
be a binary mask, with $\beta_i$
indicates whether the $i$-th neuron should be split ($\beta_i=1$) or not ($\beta_i=0$).
The task of choosing a optimal subset to split is equivalent to search the optimal combination of $\{\beta_i\}$ that minimizes the total loss decrease via splitting:
$$
\min_{\vv\beta} \sum_{\ell=1}^n \beta_\ell \lambda_{\min}^\ell, ~~~\text{s.t.}~~\sum_\ell \beta_\ell = c, \beta_\ell \in\{0, 1\},
$$
where $\beta_{\min}^\ell$ stands for the splitting index of the $\ell$-th neuron and $c$ is the maximum number of neurons to split.
% \paragraph{Growing neural network via splitting}
% In practice, the generalization works by splitting existing neurons 
% into multiple copies thus discovering novel architectures. 
% % In the perspective of neural architecture optimization, the aforementioned generalization
% % corresponds to introduce more neurons thus growing the network. 
% % \paragraph{Deriving optimal splitting}


% Consider a $d$-layer neural networks, 
% let $\Theta= [\{\theta_i^{[1]}\}_{i=1}^{m_1}, \cdots, \{\theta_i^{[d]}\}_{i=1}^{m_d}]$ be the collection of model parameters of the network, with $\{\theta_i^{[\ell]}\}_{i=1}^{m_\ell}$ as the neurons in the $\ell$-th layer and $m_\ell$ the number of neurons.

% Given a set of training data $\gD=\{(x, y)\}$,
% we train the network by minimizing the empirical risk,
% $$
% \min_{\Theta} \E_{x, y \sim \gD} ~~\gL(x, y; \Theta),
% $$
% where $\ell(\cdot)$ denotes the loss function.
% At stable local minima, the first order gradients
% become zero and no furhter imporovement can be made. 


% % \begin{align*}
% %     &\min_{\rho} ~~~\gL(\hat{\rho}^{(k)}) - \gL(\rho^{(k)}) \\
% %     & ~s.t.  ~~ W(\hat{\rho}_i, \rho_i) \le \epsilon, ~~~\forall i \\
% %     & ~~~~~ \sum_{i=1}^k \bigg(F[\hat{\rho}_i] - F[\rho_i]  \bigg) \le \tau 
% % \end{align*}

% % In this paper, we restrict the

% % \begin{align*}
% % \min_z ~~\gL(\Phi(\rho, z)) - \gL(\rho) \\
% % \text{s.t.}~~ \gR(\Phi(\rho, z)) - \gR(\rho) \le \tau\\
% % z_i \in \{0, 1\} ~~\forall i \\
% % \end{align*}


% Consider split each neuron $\theta \in \Theta$ into to 
% $m$ coipies, $\{w_i, \theta_i\}$, 
% xx show


% And the optimal spitting striegies would be


% Following xx, for each neuron xx, we split into $k$ copyies,
% with a update rule
% $$
% \theta_i^{[\ell]} = \theta^{[\ell]} + \epsilon(v + v_i), ~~\text{s.t.}~~~ \sum_i v_i = 1.
% $$



% Let $\rho$ is a distributiuon that parameterized the neural network of xxx
% where $F[\rho]$ denotes the neural network


% In practice, 
% \cipte{xx} suggests to the split the top $xx$ neurons with the smallest spliting-index
% according to the optimal splitting relu~\eqref{xxx}.
 


\section{Energy-aware Splitting}
\label{sec:energy-splitting}

The aforementioned approach grows the network that only focusing on
empirical loss minimization 
while neglecting the different energy consumption of different neurons. 
Intuitively, one may consider using less neurons in shallow layers (close to inputs)
which have larger input resolution and consume more energy in general; 
on the other hand, one should retain more neurons in deep layers which are responsible for final classification and computational cheap.  
The splitting strategy contributes to the final accuracy and energy efficiency of neural architectures in a complex manner. 


% Let $\vv\beta$ be a binary mask, with each element $\beta_i$ indicautes whether the $i$-th  neuron should be split ($\beta_i=1$) or not ($\beta_i=0$).
We formulate the problem of searching energy-efficient networks as a constrained optimization problem,  by finding the optimal 
splitting strategy such that the loss is maximumly decreased 
under an energy constrain. More specifilay, out splitting process solves,
% We further propose an energy-aware splitting mechanism that 
% allows us to learn more resource-efficient networks. 
% Similarly, we could formulate this into the following optimization problem,
% In this paper, we restrict the
\begin{align*}
&\min_{\vv\beta} \sum_{\ell=1}^n \beta_\ell \lambda_{\min}^\ell, \\
& ~~~\text{s.t.}~~~~\gR(\vv\beta) \le (1+\alpha) \gR(\vv 0)\\
% &\min_{\vv\beta} ~~\gL(\Phi(\rho, \vv\beta)) - \gL(\rho) \\
% &\text{s.t.}~~ \gR(\Phi(\rho, \vv\beta)) \le (1 + \alpha)\gR(\rho)  \\
&~~~\beta_i \in \{0, 1\}, ~~\forall i \\
\end{align*}
where  $\gR(\vv\beta)$ measures the additional energy-cost introduced if we grew the network according to the splitting mask $\vv \beta$, $\gR(\vv 0)$ represents the energy cost of the previous network without splitting, 
and $\alpha \in [0, 1]$ control the growth ratio for each splitting process.

\red{QL: Elaborate how we can measure $R(
\beta)$ here? Do you assume each neuron has a cost of $c_i$, andd$R(\beta)$ is the sum of it?}

\red{QL: we should point out that this is a knapsack problem and discuss how we will solve it (NP-hardness, greedy algorithm, or convex relaxation)  \url{https://en.wikipedia.org/wiki/Knapsack_problem}}

\red{QL: solving it how fastly? make the point that we do not need to solve this problem to high accruacy, because parameters are noisy anyway. }




%Given a budget of growing the network with $c$ neurons, we should choose the the best subset of neurons that maximize the decrease loss.
% The splitting effects of different neurons can be compared using the optimal% individual gain (see Eq.\eqref{eq:loss_decrease}) without considering the other neurons.% allowing us to decide the bes% subset of neurons to split when a maximum number constrain is imposed.
%To be precise, we demote by $\lambda_{\min}(i)$ the gain via splitting the $i$-th neuron.
% and $c_i$ the estimated cost of splitting 
% the $i$-th neuron from the current network.
% To be precise,
%For a neural network with $n$ neurons, let $\vv\beta \in \R^n$be a binary mask, with $\beta_i$indicates whether the $i$-th neuron should be split ($\beta_i=1$) or not ($\beta_i=0$).The task of choosing an optimal subset to split is equivalent to search the optimal combination of $\{\beta_i\}$ that minimizes the total loss decrease via splitting:
%\begin{align}\min_{\vv\beta} \sum_{i=1}^n \beta_i \lambda_{\min}(i), ~~~\text{s.t.}~~\sum_{i=1}^n \beta_i = c, ~\beta_i \in\{0, 1\}, \forall i.\label{eq:splitting_opt}\end{align}
% where $\beta_{\min}^\ell$ stands for the splitting index of the $\ell$-th neuron and $c$ is the maximum number of neurons to split.

The method above allows us to select the best subset of neurons to split to yield the steepest descent on the loss function. 
%However, in practice settings, splitting different neurons can cause significantly different  and 
%grow the networks yield the
%The splitting process allows us to grow the network,thus yielding a framework for implicit neural architecture space exploration.
%However, the approach above 
%expands the network that is only focusing onempirical loss minimization 
In practice, however, 
splitting different neurons incurs a different amount of increase on the model size,  computational cost, and physical energy consumption. For example, 
splitting a neuron connecting to a large number of inputs and outputs increases the size and computational cost of the network much more significantly than splitting the neurons with less inputs and outputs.
%while neglecting the different energy consumption of different neurons. 
Intuitively, one may want to split fewer neurons in layers close to inputs, which typically have larger input resolutions and a high energy cost, while split more neurons in deep layers which are responsible for the final classification and have lower computational cost.   
A better splitting strategy should consider taking the different cost of splitting different neurons into account. 
%influence of the loss in a 
%to the final accuracy and energy efficiency in a complex manner. 

To address this problem, we propose to explicitly  incorporate the  splitting cost different neurons 
to better guide the splitting process.
Specifically, we 
propose to decide the optimal splitting set by solving the following constrained optimization: 
% Let $\vv\beta$ be a binary mask, with each element $\beta_i$ indicautes whether the $i$-th  neuron should be split ($\beta_i=1$) or not ($\beta_i=0$).
% To be precision, we formulate the problem of searching energy-efficient networks as a constrained optimization problem,  by finding the optimal 
% splitting strategy such that the loss is maximumly decreased 
% under an energy constrain. 
% More specifilay, out splitting process solves,
% We further propose an energy-aware splitting mechanism that 
% allows us to learn more resource-efficient networks. 
% Similarly, we could formulate this into the following optimization problem,
% In this paper, we restrict the
\begin{align}
\min_{\vv \beta} \sum_{\ell=1}^n \beta_\ell \lambda_{\min}(\ell),~~
\sum_{\ell=1}^n e_\ell \beta_\ell \le e_{budget}, 
% & ~~~\text{s.t.}~~~~\gR(\vv\beta) \le (1+\alpha) \gR(\vv 0)\\
% &\min_{\vv\beta} ~~\gL(\Phi(\rho, \vv\beta)) - \gL(\rho) \\
% &\text{s.t.}~~ \gR(\Phi(\rho, \vv\beta)) \le (1 + \alpha)\gR(\rho)  \\
~~~\beta_\ell \in \{0, 1\}, ~~\forall \ell, 
\label{eq:energy_aware_splitting}
\end{align}
where $\beta_\ell$ denotes if enuron $i$ should be split, and 
$e_\ell$ represents the cost of splitting neuron $i$ at the current iteration of splitting steepest descent. 
%Note that $$
% where  $\gR(\vv\beta)$ measures the additional energy-cost introduced if we grew the network according to the splitting mask $\vv \beta$, $\gR(\vv 0)$ represents the energy cost of the previous network without splitting, 
% and $\alpha \in [0, 1]$ control the growth ratio for each splitting process.
In this work, we take $e_\ell$ to be  energy cost, measured by 
flops.  
Note that the cost of splitting the same neuron changes across iterations as the network topology changes. Therefore, we re-evaluate the cost of every neuron at each network growing stage, based on the topology of the current network. See  Algorithm~\ref{alg:main} for an overview of our method.

Specifically, consider a 2D convolutional layer with filters of size $k\times k$.
Let $H$ be the total number 
